Resolved Neutral Outflow from a Lensed Dusty Star Forming Galaxy at z=2.09

We report the detection of a massive neutral gas outflow in the z=2.09 gravitationally lensed Dusty Star-Forming Galaxy HATLASJ085358.9+015537 (G09v1.40), seen in absorption with the OH+(1_1-1_0) transition using spatially resolved (0.5"x0.4") Atacama Large Millimeter/submillimeter Array (ALMA) observations. The blueshifted OH+ line is observed simultaneously with the CO(9-8) emission line and underlying dust continuum. These data are complemented by high angular resolution (0.17"x0.13") ALMA observations of CH+(1-0) and underlying dust continuum, and Keck 2.2 micron imaging tracing the stellar emission. The neutral outflow, dust, dense molecular gas and stars all show spatial offsets from each other. The total atomic gas mass of the observed outflow is 6.7x10^9 M_sun, >25% as massive as the gas mass of the galaxy. We find that a conical outflow geometry best describes the OH+ kinematics and morphology and derive deprojected outflow properties as functions of possible inclination (0.38 deg-64 deg). The neutral gas mass outflow rate is between 83-25400 M_sun/yr, exceeding the star formation rate (788+/-300 M_sun/yr) if the inclination is >3.6 deg (mass-loading factor = 0.3-4.7). Kinetic energy and momentum fluxes span 4.4-290x10^9 L_sun and 0.1-3.7x10^37 dyne, respectively (energy-loading factor = 0.013-16), indicating that the feedback mechanisms required to drive the outflow depend on the inclination assumed. We derive a gas depletion time between 29 and 1 Myr, but find that the neutral outflow is likely to remain bound to the galaxy, unless the inclination is small, and may be re-accreted if additional feedback processes do not occur.

==> hyphens.tex <==
\hyphenation{ASTRON}                    % how to (not) break these words
\hyphenation{cloud-let cloud-lets}
\hyphenation{HVABG}
\hyphenation{MNRAS}
\hyphenation{Peim-bert}
\hyphenation{Schloerb}
\endinput


==> journals.tex <==
\def\jltp{J.~Low Temp.\ Phys.}
\def\natas{Nature Astronomy}
\def\rmxaa{Rev.\ Mex.\ Astron.\ Astr.}

\endinput


==> molec.tex <==
%--------------- molecules and molecular ions --------------------------------
%

\def\mbox{\hbox}           % for compatibility of TeX and LaTeX use 

\def\CHp{\ifmmode \mbox{\rm CH}^+           %   +
         \else {\rm CH}$^+$                 % CH
         \fi}

\def\CO#1{\ifnum#1=0                    % CO isotopes
           \ifmmode \mbox{\rm CO}
           \else {\rm CO}
           \fi
          \else
           \ifnum#1<15
            \ifmmode ^{#1}\mbox{\rm CO}
            \else $^{#1}${\rm CO}
            \fi
           \else
            \ifmmode \mbox{\rm C}^{#1}\mbox{\rm O}
            \else {\rm C}$^{#1}${\rm O}
            \fi
           \fi
          \fi}

\def\COp{\ifmmode \mbox{\rm CO}^+           %   +
         \else {\rm CO}$^+$                 % CO
         \fi}

\def\CS#1{\ifnum#1=0                    % CS isotopes
           \ifmmode \mbox{\rm CS}
           \else {\rm CS}
           \fi
          \else
           \ifnum#1<15
            \ifmmode ^{#1}\mbox{\rm CS}
            \else $^{#1}${\rm CS}
            \fi
           \else
            \ifmmode \mbox{\rm C}^{#1}\mbox{\rm S}
            \else {\rm C}$^{#1}${\rm S}
            \fi
           \fi
          \fi}

\def\HCOp{\ifmmode \mbox{\rm HCO}^+          %    +
          \else {\rm HCO}$^+$                % HCO
          \fi}

\def\HCtN{\ifmmode \mbox{\rm HC}_3\mbox{\rm N}     % HC N
          \else {\rm HC}$_3${\rm N}                %   3
          \fi}

\def\Hp{\ifmmode \mbox{\rm H}^+           %  +
        \else {\rm H}$^+$                 % H
        \fi}
                                                  %    +
\def\HtOp{\ifmmode \mbox{\rm H}_2\mbox{\rm O}^+   % H O
          \else {\rm H}$_2${\rm O}$^+$            %  2
          \fi}
                                                   %    +
\def\HthOp{\ifmmode \mbox{\rm H}_3\mbox{\rm O}^+   % H O
              \else {\rm H}$_3${\rm O}$^+$         %  3
              \fi}
                                            %  +
\def\Hthp{\ifmmode \mbox{\rm H}_3^+         % H
             \else {\rm H}$_3^+$            %  3
             \fi}

\def\Ht{\ifmmode \mbox{\rm H}_2              % H
        \else {\rm H}$_2$                    %  2
        \fi}

\def\HtCO{\ifmmode \mbox{\rm H}_2\mbox{\rm CO} % H CO
          \else {\rm H}$_2${\rm CO}            %  2
          \fi}

\def\HtO{\ifmmode \mbox{\rm H}_2\mbox{\rm O} % H O
         \else {\rm H}$_2${\rm O}            %  2
         \fi}
                                                   %  18
\def\HteO{\ifmmode \mbox{\rm H}_2^{18}\mbox{\rm O} % H O
          \else {\rm H}$_2^{18}${\rm O}            %  2
          \fi}

\def\OHp{\ifmmode \mbox{\rm OH}^+   %   +
         \else {\rm OH}$^+$         % OH
         \fi}

\def\NHt{\ifmmode \mbox{\rm NH}_3            % NH
         \else {\rm NH}$_3$                  %   3
         \fi}

\def\NHtw{\ifmmode \mbox{\rm NH}_2            % NH
          \else {\rm NH}$_2$                  %   2
          \fi}

%
%---------------------- atoms and atomic ions ---------------------------------
%

\def\ion#1#2{\ifmmode \mbox{{\rm #1}}\,\mbox{{\sc #2}} % generic ion
        \else {\rm #1}$\,${\sc #2}
        \fi}
\def\CI{\ion{C}{i}}
\def\CII{\ion{C}{ii}}
\def\FeII{\ion{Fe}{ii}}
\def\HI{\ion{H}{i}}
\def\HII{\ion{H}{ii}}
\def\NII{\ion{N}{ii}}
\def\NeII{\ion{Ne}{ii}}
\def\OI{\ion{O}{i}}
\def\OII{\ion{O}{ii}}
\def\OIII{\ion{O}{iii}}
\def\SII{\ion{S}{ii}}
\def\SIII{\ion{S}{iii}}
\def\SiII{\ion{Si}{ii}}
\def\SiVI{\ion{Si}{vi}}

%
%-------------------- hydrogen recombination lines ---------------------------
%

\def\rec#1#2{\if#2a                            % generic
              \ifmmode \mbox{{\rm #1}}\alpha   % recombination line
              \else {\rm #1}$\alpha$
              \fi
             \fi
             \if#2b
              \ifmmode \mbox{{\rm #1}}\beta
              \else {\rm #1}$\beta$
              \fi
             \fi
             \if#2g
              \ifmmode \mbox{{\rm #1}}\gamma
              \else {\rm #1}$\gamma$
              \fi
             \fi}

\def\Lya{\rec{Ly}{a}}                          % Lyman alpha
\def\Ha{\rec{H}{a}}                            % H alpha
\def\Hb{\rec{H}{b}}                            % H beta
\def\Paa{\rec{Pa}{a}}                          % Paschen alpha
\def\Pab{\rec{Pa}{b}}                          % Paschen beta
\def\Bra{\rec{Br}{a}}                          % Brackett alpha
\def\Brg{\rec{Br}{g}}                          % Brackett gamma

\endinput


==> refs.tex <==
%..............................................................................
%
%             This is    r e f s . t e x
%
% A LaTeX file for keeping tracks of references to figures, sections,
% tables and equations.
%
% Latest update: PvdW 12-Sep-2016 removed \eqref for compatibility with amstex
%
%..............................................................................

\newcommand{\tabref}[1]{Table~\protect\ref{#1}}
\newcommand{\figref}[1]{Fig.~\protect\ref{#1}}
\newcommand{\figrefbare}[1]{\protect\ref{#1}}
\newcommand{\figrefs}[1]{Figs.~\protect\ref{#1}}
\newcommand{\figsref}[2]{Figs.~\protect\ref{#1}--\protect\ref{#2}}
\newcommand{\twofigsref}[2]{Figs.~\protect\ref{#1} and~\protect\ref{#2}}
%\newcommand{\eqref}[1]{Eq.~$\left(\protect\ref{#1}\right)$}
\newcommand{\eqsref}[2]{Eqs.~$\left(\protect\ref{#1}\right)$--$\left(\protect\ref{#2}\right)$}
\newcommand{\twoeqsref}[2]{Eqs.~$\left(\protect\ref{#1}\right)$--$\left(\protect\ref{#2}\right)$}
\newcommand{\secref}[1]{Sect.~\protect\ref{#1}}
\newcommand{\secsref}[2]{Sects.~\protect\ref{#1}--\protect\ref{#2}}
\newcommand{\twosecsref}[2]{Sects.~\protect\ref{#1} and~\protect\ref{#2}}

% upper case versions to begin sentences: 

\newcommand{\Tabref}[1]{\tabref{#1}}
\newcommand{\Figref}[1]{Figure~\protect\ref{#1}}
\newcommand{\Figrefs}[1]{Figures~\protect\refs{#1}}
\newcommand{\Figsref}[2]{Figures~\protect\ref{#1}--\protect\ref{#2}}
\newcommand{\Eqref}[1]{Equation~(\protect\ref{#1})}
\newcommand{\Eqsref}[2]{Equations~(\protect\ref{#1})--(\protect\ref{#2})}
\newcommand{\Secref}[1]{Section~\protect\ref{#1}}

\endinput


==> symbols.tex <==
\def\mbox{\hbox}           % for compatibility of TeX and LaTeX use

%------------------ degrees, magnitudes, RA, Dec etc -------------------------
%

\def\deg{\ifmmode ^\circ                % degrees symbol
         \else $^\circ$
         \fi
         \hskip -0.1truecm}
\def\degd#1.#2{                         % degrees over decimal point
                                        % syntax: \degd 4.3 or \degd 4.{34}
               \ifmmode {#1^{\hskip 0.05em\circ}\hskip-0.42em.\hskip0.08em#2}
               \else {#1$^{\hskip 0.05em\circ}\hskip-0.42em.\hskip0.08em$#2}
               \fi
              }
\def\mind#1.#2{                         % minutes over decimal point
                                        % syntax: \mind 4.3
               \ifmmode {#1^{\hskip 0.05em\prime}\hskip-0.35em.\hskip0.05em#2}
               \else {#1$^{\hskip 0.05em\prime}\hskip-0.35em.\hskip0.05em$#2}
               \fi
              }
\def\secd#1.#2{                         % seconds over decimal point
                                        % syntax: \secd 4.3
               \ifmmode {#1^{\prime\prime}\hskip-0.46em.\hskip0.12em#2}
               \else {#1$^{\prime\prime}\hskip-0.46em.\hskip0.12em$#2}
               \fi
              }
\def\timsecd#1.#2{                      % time seconds over decimal point
                                        % syntax: \timsecd 4.3
                  \ifmmode {#1^{\rm s}\hskip-0.39em.\hskip0.08em#2}
                  \else {$#1^{\rm s}\hskip-0.39em.\hskip0.08em#2$}
                  \fi
                 }
\def\hms#1h#2m#3s{                      % hms format (for RA)
                                        % syntax: \hms 12h34m45s
                  \relax
                  \ifmmode #1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}
                  \else \hbox{$#1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}$}
                  \fi
                 }
\def\dms#1d#2m#3s{                      % dms format (for Dec)
                                        % syntax: \dms 12d14m45s
                  \relax
                  \ifmmode #1^\circ\,#2^{\prime}\,#3^{\prime\prime}
                  \else \hbox{$#1^\circ\,#2^{\prime}\,#3^{\prime\prime}$}
                  \fi
                 }
\def\dmsd#1d#2m#3.#4s{                  % dms format with decimal point (Dec)
                                        % syntax: \dmsd 12d13m34.5s
                      \relax
                      \ifmmode #1^\circ\,#2^{\prime}\,#3^{\prime\prime}
                               \hskip-0.46em.\hskip0.12em#4
                      \else \hbox{$#1^\circ\,#2^{\prime}\,#3^{\prime\prime}
                            \hskip-0.46em.\hskip0.12em#4$}
                      \fi
                     }
\def\hm#1h#2m{                          % hm format (for RA)
                                        % syntax: \hm 12h13m
              \relax
              \ifmmode #1^{\rm h}\,#2^{\rm m}
              \else \hbox{$#1^{\rm h}\,#2^{\rm m}$}
              \fi
             }
\def\dm#1d#2m{                          % dm format (for Dec)
                                        % syntax: \dm 12d13m
              \relax
              \ifmmode #1^\circ\,#2^{\prime}
              \else \hbox{$#1^\circ\,#2^{\prime}$}
              \fi
             }
\def\hmsd#1h#2m#3.#4s{                  % hms format with decimal point (RA)
                                        % syntax: \hmsd 12h13m34.5s
                      \relax
                      \ifmmode #1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}
                               \hskip-0.39em.\hskip0.08em#4
                      \else \hbox{$#1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}
                            \hskip-0.39em.\hskip0.08em#4$}
                      \fi
                     }
\def\hmd#1h#2.#3m{                  % hm format with decimal point (RA)
                                    % syntax: \hmd 12h13.6m
                  \relax
                  \ifmmode #1^{\rm h}\,#2^{\rm m}
                           \hskip-0.55em.\hskip0.22em#3
                  \else \hbox{$#1^{\rm h}\,#2^{\rm m}
                        \hskip-0.55em.\hskip0.22em#3$}
                  \fi
                 }
\def\mg{\relax                          % magnitudes symbol
        \ifmmode ^{\rm m}
        \else $^{\rm m}$
        \fi
       }
\def\mgd#1.#2{                          % magnitudes over decimal point
                                        % syntax: \mgd 4.3
              \relax
              \ifmmode #1^{\rm m}
                       \hskip-0.55em.\hskip0.22em#2
              \else \hbox{#1$^{\rm m}
                    \hskip-0.55em.\hskip0.22em$#2}
              \fi
             }

%
%-------------------- math symbols --------------------------------------------
%

\def\la{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\ga{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}

%
%--------------------------- units -------------------------------------------
% use: e.g. $15\kms$
%

\def\unitspace{\;}                      % space to be used with units

\def\un#1{\ifmmode \unitspace\mbox{\rm #1} % generic unit
          \else $\unitspace$#1
          \fi}
\def\pun#1#2{\ifmmode \unitspace\mbox{\rm #1}^{#2} % generic unit with a power
             \else $\unitspace$#1$^{#2}$
             \fi}
\def\per#1{\ifmmode \unitspace\mbox{\rm #1}^{-1} % generic unit with power -1
           \else $\unitspace$#1$^{-1}$
           \fi}

\def\Ang{\un{\AA}}                    % Angstrom
\def\AU{\un{AU}}                      % AU
\def\cm{\un{cm}}                      % cm
\def\es{\un{erg}\ps}                  %      -1
                                      % erg s
\def\esc{\es\pcmsqu}                  %      -1 -2
                                      % erg s cm
\def\escmum{\esc\mum^{-1}}            %      -1 -2  -1
                                      % erg s cm  mu
\def\escs{\esc\pun{sr}{-1}}           %      -1 -2 -1
                                      % erg s cm sr
\def\escsm{\escs\mum^{-1}}            %      -1 -2 -1 -1
                                      % erg s cm sr mu
\def\Eu{\font\euro = eurorm {\euro E}} % Euro
\def\eV{\un{eV}}                      % eV
\def\GHz{\un{GHz}}                    % GHz
\def\Jy{\un{Jy}}                      % Jy
\def\K{\un{K}}                        % K
\def\kms{\un{km}\pun{s}{-1}}          %     -1
                                      % km s
\def\kpc{\un{kpc}}                    % kpc
\def\Lsun{\ifmmode \un{L}_{\odot}     % solar luminosity
          \else $\un{L}_{\odot}$
          \fi}
\def\MHz{\un{MHz}}                    % MHz
\def\mJy{\un{mJy}}                    % mJy
\def\mm{\un{mm}}                      % mm
\def\Mpc{\un{Mpc}}                    % Mpc
\def\Msun{\ifmmode \un{M}_{\odot}     % solar mass
          \else $\un{M}_{\odot}$
          \fi}
\def\muJy{\ifmmode \unitspace\mu\mbox{\rm Jy} % microJansky
          \else $\unitspace\mu$Jy
          \fi}
\def\mum{\ifmmode \unitspace\mu\mbox{\rm m} % micron
         \else $\unitspace\mu$m
         \fi}
\def\nm{\un{nm}}                      % nm
\def\pc{\un{pc}}                      % pc
\def\pcm{\per{cm}}                    %   -1
                                      % cm
\def\pcmcub{\pun{cm}{-3}}             %   -3
                                      % cm
\def\pcmsqu{\pun{cm}{-2}}             %   -2
                                      % cm
\def\pyr{\pun{yr}{-1}}                %   -1
                                      % yr
\def\ps{\pun{s}{-1}}                  %  -1
                                      % s
\def\sqarcsec{\ifmmode \unitspace\Box''    %       2
              \else $\unitspace\Box''$     % arcsec
              \fi} 

%
%-------------------------- quantities ---------------------------------------
%

\def\Bp{\relax                            % B
        \ifmmode B_{||}                   %  ||
        \else $B_{||}$
        \fi}
\def\Bt{\relax                            % B
        \ifmmode B\!_{\perp}              %  |
        \else $B\!_{\perp}$               %  -
        \fi}
\def\Dec{\relax                           % Dec
          \ifmmode \mbox{\rm Dec}
          \else Dec
         \fi}
\def\Eup{\relax                           % E
         \ifmmode E_{\rm u}               %  u
         \else $E_{\rm u}$
         \fi}
\def\Gcr{\relax                           % Gamma
         \ifmmode \Gamma\!_{\rm cr}       %      cr
         \else $\Gamma\!_{\rm cr}$
         \fi}
\def\ICII{\relax                          % I
          \ifmmode I_{[\CII]}             %  [C II]
          \else $I_{[\CII]}$
          \fi}
\def\LHtwo{\relax                                 % L
           \ifmmode L_{\mbox{\rm\scriptsize H}_2} %  H
           \else $L_{\mbox{\rm\scriptsize H}_2}$  %   2
           \fi}
\def\LFIR{\relax                           % L
          \ifmmode L_{\rm FIR}             %  FIR
          \else $L_{\rm FIR}$
          \fi}
\def\LIR{\relax                           % L
         \ifmmode L_{\rm IR}              %  IR
         \else $L_{\rm IR}$
         \fi}
\def\LLya{\relax                          % L
          \ifmmode L_{{\rm Ly}\,\alpha}   %  Ly alpha
          \else $L_{{\rm Ly}\,\alpha}$
          \fi}
\def\mAB{\relax                           % m
         \ifmmode m_{\rm AB}              %  AB
         \else $m_{\rm AB}$
         \fi}
\def\mHI{\relax                                      % m
         \ifmmode m_{\mbox{\scriptsize\rm H\,\sc I}} %  HI
         \else $m_{\mbox{\scriptsize\rm H\,\sc I}}$
         \fi}
\def\MHII{\relax                                       % M
          \ifmmode M_{\mbox{\scriptsize\rm H\,\sc II}} %  HII
          \else $M_{\mbox{\scriptsize\rm H\,\sc II}}$
          \fi}
\def\MHtwo{\relax                                 % M
           \ifmmode M_{\mbox{\rm\scriptsize H}_2} %  H
           \else $M_{\mbox{\rm\scriptsize H}_2}$  %   2
           \fi}
\def\MHtwodot{\relax                                       % .
              \ifmmode \dot{M}_{\mbox{\rm\scriptsize H}_2} % M
              \else $\dot{M}_{\mbox{\rm\scriptsize H}_2}$  %  H
              \fi}                                         %   2
\def\Mstardot{\relax                      % .
              \ifmmode \dot{M}_{\ast}     % M
              \else $\dot{M}_{\ast}$      %  *
              \fi}
\def\nH{\relax                                       % n
        \ifmmode n_{\mbox{\scriptsize\rm H}}  %  H
        \else $n_{\mbox{\scriptsize\rm H}}$
        \fi}
\def\nHI{\relax                                      % n
         \ifmmode n_{\mbox{\scriptsize\rm H\,\sc I}} %  HI
         \else $n_{\mbox{\scriptsize\rm H\,\sc I}}$
         \fi}
\def\nHt{\relax                                % n
         \ifmmode n_{{\mbox{\scriptsize H}}_2} %  H
         \else $n_{{\mbox{\scriptsize H}}_2}$  %   2
         \fi}
\def\RA{\relax                           % RA
         \ifmmode \mbox{\rm RA}
         \else RA
        \fi}
\def\rhostardot{\relax                         %  .
                \ifmmode \dot{\rho}_{\ast}     % rho
                \else $\dot{\rho}_{\ast}$      %    *
                \fi}
\def\rhoZdot{\relax                          %  .
             \ifmmode \dot{\rho}_{\rm Z}     % rho
             \else $\dot{\rho}_{\rm Z}$      %    Z
             \fi}
\def\Tb{\relax                           % T
        \ifmmode T_{\rm b}               %  b
        \else $T_{\rm b}$
        \fi}
\def\Tc{\relax                           % T
        \ifmmode T_{\rm c}               %  c
        \else $T_{\rm c}$
        \fi}
\def\Td{\relax                           % T
        \ifmmode T_{\rm d}               %  d
        \else $T_{\rm d}$
        \fi}
\def\Te{\relax                           % T
        \ifmmode T_{\rm e}               %  e
        \else $T_{\rm e}$
        \fi}
\def\Tg{\relax                           % T
        \ifmmode T_{\rm g}               %  g
        \else $T_{\rm g}$
        \fi}
\def\Tkin{\relax                         % T
          \ifmmode T_{\rm kin}           %  kin
          \else $T_{\rm kin}$
          \fi}
\def\Ts{\relax                           % T
        \ifmmode T_{\rm s}               %  s
        \else $T_{\rm s}$
        \fi}
\def\vhel{\relax                  %
          \ifmmode \qu{v}{hel}    % v
          \else $\qu{v}{hel}$     %  hel
          \fi}
\def\vLSR{\relax                  %
          \ifmmode \qu{v}{LSR}    % v
          \else $\qu{v}{LSR}$     %  LSR
          \fi}

%
%------------------ source designations -------------------------
%

\def\sou#1#2{\relax                       % source designations
             \ifmmode {\rm #1}\,{\rm #2}  % e.g. \sou{Arp}{220}
             \else #1$\,$#2
             \fi}

\def\APM#1{\sou{APM}{#1}}                % APM number

\def\Arp#1{\sou{Arp}{#1}}                % Arp number

\def\HD#1{\sou{HD}{#1}}                  % HD number

\def\HH#1{\sou{HH}{#1}}                  % HH number

\def\IC#1{\sou{IC}{#1}}                  % IC number

\def\IRAS#1{\sou{IRAS}{#1}}              % IRAS number

\def\Mrk#1{\sou{Mrk}{#1}}                % Mrk number

\def\NGC#1{\sou{NGC}{#1}}                % NGC number

\def\SMM#1{\sou{SMM}{#1}}                % SMM number

\def\UGC#1{\sou{UGC}{#1}}                % UGC number

%
%------------------- generic quantity symbols ------------------
%

\def\qu#1#2{\relax                          % quantity symbols
            \ifmmode #1_{\rm #2}            % e.g. \qu{L}{FIR}
            \else $#1_{\rm #2}$
            \fi}

\endinput

